Interactions in Higher-Spin Gravity: a Holographic Perspective

This thesis is an elaboration of recent results on the holographic re-construction of metric-like interactions in higher-spin gauge theories on anti-de Sitter space (AdS), employing their conjectured holographic duality with free conformal field theories (CFTs). After reviewing the general approach and establishing the necessary intermediate results, we extract explicit expressions for the complete cubic action on AdS$_{d+1}$ and the quartic self-interaction of the scalar on AdS$_4$ for the type A minimal bosonic higher-spin theory from the three- and four- point correlation functions of single-trace operators in the free scalar $O\left(N\right)$ vector model. For this purpose tools were developed to evaluate tree-level three-point Witten diagrams involving fields of arbitrary integer spin and the conformal partial wave expansions of tree-level four-point Witten diagrams, which are underpinned by the ambient space formulation of AdS space and CFT. We also discuss the implications of the holographic duality on the locality properties of interactions in higher-spin gauge theories.

==> abstract.tex <==
\addcontentsline{toc}{chapter}{\protect Abstract}


This thesis is an elaboration on recent results on the (holographic) re-construction of interactions in higher-spin gauge theories on anti-de Sitter space (AdS)  using their conjectured duality with free conformal field theories. We demonstrate how the complete cubic action and the quartic self-interactions of the scalar in the type A minimal bosonic higher-spin theory on AdS$_{d+1}$ can be extracted from the correlation functions of single-trace operators in the free scalar $O\left(N\right)$ vector model.






\thispagestyle{empty}

\vspace*{1cm}

\noindent
\textcolor{nicegray}{{\bf \sffamily \huge Abstract}}
\vspace*{1cm}

In this thesis we investigate aspects of higher-spin gravity on an anti-de Sitter (AdS) background.
Such theories are believed to give an effective description of quantum gravity in its high energy regime, where there have been hints that a large underlying (higher-spin) symmetry may become restored. The possibility of this behaviour gained plausibility through considerations of string theory in the high-energy (tensionless) limit. The study of higher-spin gauge theories is thus of relevance, in particular for their infinite dimensional symmetry may serve as a guiding principle to help shed light on the nature of quantum gravity at energies which are beyond the reach of present day experiments. \\


To fulfil this potential, there is much still to be understood about higher-spin theories themselves. To date, the fully non-linear formulations of higher-spin theories include infinitely many additional auxiliary fields. In this work we take steps towards clarifying the nature of interactions amongst higher-spin fields in a metric-like Lagrangian framework, free from such auxiliary fields. To this end, we employ the conjectured holographic duality between higher-spin gravity theories on AdS and certain, solvable, conformal field theories (CFTs). In this way well-known methods in CFT may be applied, and with them we determine completely all cubic interactions and the quartic self-interaction of the scalar in the higher-spin Lagrangian on an AdS background. For this purpose a number of further original results were established, which include: Tools to evaluate three-point amplitudes in AdS space involving external fields of arbitrary integer spin, propagators for gauge fields of arbitrary integer spin on an AdS background, and techniques to determine conformal partial wave expansions of four-point amplitudes in higher-spin theories. 
\\


Reminiscent of the tail of $\alpha^\prime$ corrections in string theory, higher-spin interactions are non-local in the sense that they are unbounded in their number of derivatives. While in (finite tension) string theory this higher-derivative behaviour does not appear to pose a threat to fundamental properties like causality, in higher-spin theories this remains to be clarified. In the context of the results established in this work, we briefly discuss the implications of the AdS/CFT duality on the locality properties of interactions in higher-spin theory. In particular, by drawing on the holographic interpretation of CFT correlation functions as scattering amplitudes in the dual gravity theory on AdS. 
\\












==> zuss.tex <==
\addcontentsline{toc}{chapter}{\protect Zusammenfassung}


\thispagestyle{empty}

\vspace*{1cm}

\noindent
\textcolor{nicegray}{{\bf \sffamily \huge Zusammenfassung}}
\vspace*{1cm}

Die vorliegende Dissertation widmet sich der Untersuchung der
H\"ohere Spin-Gravitation auf einem Anti-de-Sitter-Raum (AdS).
Es gibt Hinweise darauf, dass dem 
Hochenergiebereich der Quantengravitation eine gro{\ss}e (H\"ohere Spin-) 
Symmetriegruppe 
zugrundeliegt und somit eine m\"ogliche effektive Beschreibung dieses Beriechs durch eine H\"ohere Spin-Theorie
gegeben ist.
Die Reaslisierung einer Quantengravitation mit dieser Symmetrie ist insbesondere in der String Theorie bei hohen Energien gegeben, wenn die 
Stringspannung vernachl\"assigt werden kann.


Die Untersuchung der H\"ohere Spin-Theorien ist von physikalischer Relevanz, weil ihre unendlichdimensionale Symmetrie als Leitprinzip verwendet werden kann, um neue Erkenntnisse \"uber die Quantengravitation bei Energien jenseits der heute experimentall erreichbaren Energieskalen zu gewinnen. Es muss dabei ber\"ucksichtigt werden, dass die verf\"ugbaren nichtlinearen Formulierungen der 
H\"ohere-Spin-Theorien unendlich viele Hilfsfelder mit einschlie{\ss}en, so dass selbst 
grundlegende Eigenschaften wie Unitarit\"at oder Kausalit\"at noch nicht 
vollst\"andig verstanden sind.


Zielsetzung dieser Arbeit ist es, die Wechselwirkungen zwischen 
h\"oheren Spin-Feldern im Rahmen der Lagrangeformulierung 
zu 
untersuchen, da dies ohne Hilfsfelder m\"oglich ist.
Um dies zu erm\"oglichen, wird die vermutete Dualit\"at zwischen 
der H\"ohere Spin-Gravitation im AdS-Raum 
und integrablen konformen Feldtheorien benutzt.
Durch Anwendung von Techniken der konformen 
Feldtheorie werden in der Lagrangefunktion der H\"oheren Spin-Theorie alle 
Wechselwirkungsterme bis zur dritten Ordnung sowie
die Selbstwechselwirkung des Skalarfeldes bis zur vierten Ordnung bestimmt.
Zu diesem Zweck werden neue Methoden entwickelt: 
Diese umfassen eine neue Herangehensweise zur Berechnung von Dreipunktamplituden mit externen Feldern
beliebigen Spins und die explizite Form von Propagatoren f\"ur Eichfelder mit beliebigem ganzzahligen 
Spin 
im AdS-Raum. Weiterhin werden Techniken zur Berechnung konformer partieller Wellenzerlegungen 
von Vierpunktamplituden in H\"ohere Spin-Theorien entwichelt.


Die $\alpha'$-Korrekturen in der Stringtheorie spiegeln sich in der Nichtlokalit\"at der Wechselwirkungen zwischen H\"ohere Spin-Feldern wider: Es treten beliebig hohe Ableitungen der Felder auf. In der Stringtheorie bei endlicher Stringspannung bedeuten diese h\"oheren Ableitungsterme offensichtlich keine Einschr\"ankung von fundamentalen Eigenschaften wie etwa der 
Kausalit\"at. In der H\"ohere-Spin-Theorie jedoch ist dies Gegenstand aktueller Forschung.
Im Kontext der Ergebnisse dieser Arbeit wird die Bedeutung der
AdS/CFT Dualit\"at f\"ur die Lokalit\"at der 
Wechselwirkungen zwischen H\"ohere Spin-Feldern diskutiert.
Insbesondere wird auf die holographische Interpretation der Korrelatoren in der 
konformen Feldtheorie als Streuamplituden der dualen Gravitationstheorie im AdS-Raum eingegangen.
